Heavy Flavour Physics and CP Violation at LHCb: a Ten-Year Review

Heavy flavour physics provides excellent opportunities to indirectly search for new physics at very high energy scales and to study hadron properties for deep understanding of the strong interaction. The LHCb experiment has been playing a leading role in the study of heavy flavour physics since the start of the LHC operations about ten years ago, and made a range of high-precision measurements and unexpected discoveries, which may have far-reaching implications on the field of particle physics. This review highlights a selection of the most influential physics results on CP violation, rare decays, and heavy flavour production and spectroscopy obtained by LHCb using the data collected during the first two operation periods of the LHC. The upgrade plan of LHCb and the physics prospects are also briefly discussed.

==> README <==
* Draft of review for AHEP

The template is with minimal style setting, subject to change when the journal template is available.

According to the meeting on 19/05/2021, the person responsible for each chapter is:

- Zhenwei: Introduction (introduction.tex)
- Yanxi: Heavy hadron production and spectroscopy (production.tex)
- Wenbin: CPV in b (beautyCPV.tex)
- Shanzhen: CPV in c (charmCPV.tex)
- Yuehong: Rare decays (raredecay.tex)
- Yiming: Upgrade and prospects (upgrade.tex)

Please edit the .tex file of the chapter you are assigned.
Put all the figures of that chapter in ./figs/<chapter name>, where <chapter name> is the same as your .tex file.
Use LHCb references from LHCb-xxx.bib, and non-LHCb papers as exported from INSPIRE.
Add non-LHCb entries in main.bib under your name.
Label sections as \label{sec:xxx}, similarly \label{fig:xxx} and \label{tab:xxx} for figures and tables.


